Knowledge-enhanced Black-box Attacks for Recommendations

Recent studies have shown that deep neural networks-based recommender systems are vulnerable to adversarial attacks, where attackers can inject carefully crafted fake user profiles (i.e., a set of items that fake users have interacted with) into a target recommender system to achieve malicious purposes, such as promote or demote a set of target items. Due to the security and privacy concerns, it is more practical to perform adversarial attacks under the black-box setting, where the architecture/parameters and training data of target systems cannot be easily accessed by attackers. However, generating high-quality fake user profiles under black-box setting is rather challenging with limited resources to target systems. To address this challenge, in this work, we introduce a novel strategy by leveraging items' attribute information (i.e., items' knowledge graph), which can be publicly accessible and provide rich auxiliary knowledge to enhance the generation of fake user profiles. More specifically, we propose a knowledge graph-enhanced black-box attacking framework (KGAttack) to effectively learn attacking policies through deep reinforcement learning techniques, in which knowledge graph is seamlessly integrated into hierarchical policy networks to generate fake user profiles for performing adversarial black-box attacks. Comprehensive experiments on various real-world datasets demonstrate the effectiveness of the proposed attacking framework under the black-box setting.

==> sections/model2.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}

% % \begin{document}




\subsection{An Overview of the Proposed Attacking Framework}




\begin{figure*}[ht]
\centering
\centerline{\includegraphics[width=2\columnwidth]{images/figure2_v2_cropped.pdf}}
\caption{An illustration of the proposed framework \mymodel{}. \mymodel{} consists of five major modules: profile representation learning, candidates construction, pivot selection, item picking, and injection attack and queries}
% \red{it would be better if we can explicitly show  profile representation learning, candidates construction, pivot selection, item picking, and injection attack and queries in the figure.}
\label{figure2}
\end{figure*}

%To address the problem of black-box recommendation system attacking, we propose a reinforcement learning~(RL) based method, \mymodel{}. 

The architecture of our proposed attacking framework is shown in Figure~\ref{figure2}.
The main idea of our proposed framework is to learn a best policy to achieve a long-term attack effectiveness by sequentially selecting an item from item candidates and adding it to the fake user profile, and finally inject profile into target recommender system. Specifically, at each time step $t$, for each fake user $u_i^*$, the DRL agent observes her past interactions and provides a new item $v_t$ to her fake user profile $P_{u^*_i}$. When the length of profile reaches pre-defined $T$, the agent will perform the injection attack to the target recommender system and get the reward.  %To perform the attacking under black-box setting, we adopt the DRL to.
%The actions include selecting the promising \emph{pivot} from the historical items in the fake user profile and picking the next item from the item candidates constructed based on the \emph{pivot}.%
Generally, \mymodel{} consists of four major components: attack intention learning, candidates construction, hierarchical item selection, and injection attack and queries.

The first component is \emph{Attack Intention Learning}, which aims to provide the fake user's attack intention an accurate representation $e(s_t)$. Here, $s_t$ denotes the items the fake user $u^*_i$ interacted with in $P_{u^*_i}^t=\{v_0 \rightarrow v_1 \rightarrow...\rightarrow v_{t-1}\}$ at time step $t$, which reflects the fake user's attack intention. With the power of the knowledge graph, the attack intention can be accurate represented using the knowledge level correlation in KG. Specifically, each historical item in $P_{u^*_i}^t$ aggregates its neighbor entities' embeddings via GNN, as shown in the top-left part of Figure~\ref{figure2}. Once having an accurate item representation, the attack intention $s_t$ will be further represented by RNN. Moreover, such a representation can be updated during the whole \mymodel{} training process for better attack performance.

% to incorporate the rich semantic information from KG, \mymodel{} first generates the initial embedding for each item based on the graph structure purely, then updates item embeddings via graph neural network during the whole framework training process.

To effectively promote the target item $v^*$, the items which have the same attributes as the target item are worth mining, since normal users are more likely to interact with the items with related latent semantics. Therefore, in \emph{Candidate Construction} module, rather than selecting the items from the entire item space $V$, at each time step $t$, \mymodel{} constructs the item candidates $\mathcal{C}_t$ by collecting the neighbors of historical items in $P^t_{u_i^*}$~(i.e., consider the current attack intention), and $\mathcal{C}_t$ will be served for the subsequent item selection.

% Once having the embedding of each item in the fake user profile, \mymodel{} aims to add an item to the profile sequentially to make the profile complete. However, directly selecting an item from the entire item candidates space has $O(|V|)$ possible choices. The extremely large $|V|$ leads to the sample efficiency problem for DRL~\cite{zou2019reinforcement}. To reduce the item candidates, in \emph{Candidate Construction} module, we construct the item candidates based on the correlation structure of KG. Specifically, we obtain the item candidates by collecting the neighbors of historical items in the profile being generated.
%Such correlated information not only reduces the search space but also alleviates the cold start problem.

However, collecting neighbors of all the historical items in a fake user's profile brings two problems: the item candidates size increases linearly with the profile length grows, and this manner may lead to bias. For example, items in the profile can be many hops away from the target item in KG, then incorporating the neighbors of these items will dilute the item candidates and further interferes the subsequent item selection. 
To solve these problems, In \emph{Hierarchical Item Selection} module, we adopt a hierarchical policy network. Specifically, at each time step $t$, the agent first select an \emph{anchor} item~($a_t^{(1)}$) from the current fake user profile $P_{u_i^*}^t$. We state that the neighbors of anchor item have the most contribution to the attack performance. Then, according to the fake user's attack intention $s_t$, the agent learns a policy to pick a new item~($a_2^{(2)}$) from the item candidates which consists of the neighbors of the anchor item. The new item will be added to the fake user profile.
%In this way, the size of item candidates is independent with the profile length.

% Lastly, we adopt the hierarchical policy network to first choose a "pivot" item from $P_{u^*}^t$ and then pick an item from the neighbors of "pivot". At time step $t+1$, we inject the fake user profile $P_{u^*}$ into the target system and get the reward from it. 
Lastly, in the \emph{Injection Attack and Queries} module, injection and queries are performed to attack the target recommender system by injecting the constructed fake user profile. As a result, the target system would update on the poisoned dataset. Then, queries on the spy users~(several normal users arranged in advance) in the target system are performed to obtain feedback in the form of Top-$k$ recommendations. Such feedback is then served as the reward to drive the optimization of the whole \mymodel{}
%~(i.e., updating the networks in previous components).

Next, we will introduce the attacking environment and details of all components in \mymodel{}.

\subsection{Attacking Environment}
The black-box attacking process can be formulated as a Markov decision process~(MDP) $\mathcal{<S,A,P}, r,\gamma>$ . The definition of MDP contains state space $\mathcal{S}$, action space $\mathcal{A}$, transition probability $P$, reward $r$, and discount factor $\gamma$:
\begin{enumerate}
    \item State: The state $s_t \in \mathcal{S}$ denotes the attack intention abstracted from the fake user profile $P_{u^*_i}^t=\{v_0 \rightarrow v_1 \rightarrow...\rightarrow v_{t-1}\}$ at time step $t$.
    \item Action: The action $a_t = \{a^{(1)}_t,a^{(2)}_t\} \in \mathcal{A}$ has two components. Specifically, at each time step $t$, the agent first performs the action $a_t^{(1)}$ to select an anchor item from $P_{u^*_i}^t$, then performs the action $a_t^{(2)}$ to pick a new item from the item candidates which consists of the neighbors of the anchor item.
    \item Transition probability: The state transition function $p(s_{t+1}|s_t,a_t) \in \mathcal{P}:\mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S} $ defines the probability of state transition from $s_t$ to $s_{t+1}$ when the attacker takes an action $a_t$.
    \item Reward: As the attacker aims to promote the target item $v^*$ that can be appeared in the Top-$k$ recommendation list of other users, we use the Hit Ratio~(HR@K), a ranking evaluation metric, as the reward function $r(s_t,a_t)$, which is defined as follows:

    \begin{equation}
    \begin{split}
    r(s_t,a_t) &= 
        \begin{cases}
        \sum^{|\hat{U}|}_{i=1} \text{HR}(\hat{u}_i, v^*, k)& t=T-1\\
        0& \text{otherwise}
        \end{cases}
         \\
    &\text{HR}(\hat{u}_i, v^*, k) =
    \begin{cases}
    1&v^* \in y_{\hat{u}_i,>k}\\
    0&v^* \notin y_{\hat{u}_i,>k}
    \end{cases}
    \end{split}
    \end{equation}
    where $\text{HR}(\hat{u}_i, v^*, k)$ returns the hit ratio for a target item $v^*$ in the top-$k$ list of the spy user $\hat{u}_i \in \hat{U}$. Here, the set of spy users $\hat{U}$ can be a subset of normal users who are already established in the target recommender system before the injection attack. They can be used by the attacker as a measure of promotion effectiveness of the injected fake users' profiles. We calculate the HR of each spy users after injecting the complete fake user profile with length $T$.
    \item Terminal: The attacking process will stop if the number of entire injected user profiles reaches the maximum budget $\Delta$.
    
\end{enumerate}
% For a single injection attack, we construct $N$ fake user profiles. Then, in the attacking process, at each time step $t$, the attack agent selects $N$ items $v_{i,t}, i=1,...,N$ for each fake user according to the their history interactions $P_{u^*_i}=\{v^*_0,...,v_{t-1} \}, i=1,...,N$, and get the reward $r_t$ from the target recommendation system. 
% The objective of reinforcement learning is to learn a policy $\pi:\mathcal{S \times A} \rightarrow \mathbb{R}$ that maximizes the expected discounted cumulative reward $\mathbb{E}[\sum^T_{t=0}\gamma^tr_t(s_t,a_t)]$, where $\gamma\in(0,1]$ is the discount factor.

% \paragraph{State} A state $s_t \in \mathcal{S}$ denotes the attack intention abstracted from the fake user profile $P_{u^*_i}^t=\{v_0 \rightarrow v_1 \rightarrow...\rightarrow v_{t-1}\}$ at time step $t$.

% \paragraph{Action} The action $A = \{a^{(1)}_t,a^{(2)}_t\} \in \mathcal{A}$ has two components. Specifically, at each time step $t$, the agent first performs the action $a_t^{(1)}$ to select an anchor item from $P_{u^*_i}^t$, then performs the action $a_t^{(2)}$ to pick a new item from the item candidates which consists of the neighbors of the anchor item. 
% % More specifically, the item candidates mainly contains the neighbors of $v_{a^{(1)}_t}$ based on KG. $\mathcal{A} = \{\mathcal{A}_0,...,\mathcal{A}_{T-1} \}$ is a collection of item candidates~(action space) at each time step.

% \paragraph{Transition probability} The state transition function $p(s_{t+1}|s_t,a_t) \in \mathcal{P}:\mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S} $ defines the probability of state transition from $s_t$ to $s_{t+1}$ when the attacker takes an action $a_t$.

% \paragraph{Reward} Since attacker aims to promote the target item $v^* \in V^*$ that can be appeared in the Top-$k$ list of other users, we use the Hit Ratio~(HR@K) as the ranking evaluation in reward function $r(s_t,a_t)$, which is defined as follows:

% \begin{equation}
% \begin{split}
% r(s_t,a_t) &= 
%     \begin{cases}
%     \sum^{|\hat{U}|}_{i=1} \text{HR}(\hat{u}_i, v^*, k)& t=T-1\\
%     0& \text{otherwise}
%     \end{cases}
%      \\
% &\text{HR}(\hat{u}_i, v^*, k) =
% \begin{cases}
% 1&v^* \in y_{\hat{u}_i,>k}\\
% 0&v^* \notin y_{\hat{u}_i,>k}
% \end{cases}
% \end{split}
% \end{equation}
% where $\text{HR}(\hat{u}_i, v^*_j, k)$ returns the hit ratio for a target item $v^*_j$ in the top-$k$ list of the spy user $\hat{u}_i \in \hat{U}$. Here, the set of spy users $\hat{U}$ is already established in the target recommendation system before the injection attack, which can be used by the attacker as a measure of promotion effectiveness of the injected fake users' profiles. 

% For a single injection attack, we construct $N$ fake user profiles. Then, in the attacking process, at each time step $t$, the attack agent selects $N$ items $v_{i,t}, i=1,...,N$ for each fake user according to the their history interactions $P_{u^*_i}=\{v^*_0,...,v_{t-1} \}, i=1,...,N$, and get the reward $r_t$ from the target recommendation system. 
% %When $t=T-1$, the set of profiles are injected into the target recommendation system, and the Hit Ratio will be calculated.

% \paragraph{Terminal}
% The attacking process will stop if the number of entire injected user profile reaches the maximum budget $\Delta$.

% The objective of reinforcement learning is to learn a policy $\pi:\mathcal{S \times A} \rightarrow \mathbb{R}$ that maximizes the expected discounted cumulative reward $\mathbb{E}[\sum^T_{t=0}\gamma^tr_t(s_t,a_t)]$, where $\gamma\in(0,1]$ is the discount factor.

\subsection{Knowledge-enhanced State Representation Learning}


\subsubsection{Knowledge-enhanced Item Representation learning}

KG + GNNs


\subsubsection{State Representation learning}

RNNs


% The profile representation is abstracted from the fake user's historical interacted items. 
Given a fake user profile $P_{u^*}^t = \{v_0,...,v_{t-1} \}$ with attack intention of promote an item $v*$ at time step $t$, we aim to generate its representation $e(s_t)$ to drive the DRL to optimize long-term attack effectiveness. Specifically, we first give the representation $e(v_i)$ of each item $v_i$ in the fake user profile, then generate the global representation of the attack intention $s_t$. 

% we first convert the items into embedding vectors $e(v_t) \in \mathbb{R}^{h_a}$, where $h_a$ is the dimension of the item embedding. Then, at time step $t$, according to these item embeddings, we generate the entire profile representation which can be seen as the state embedding $e(s_t)$ to drive the optimization of the whole framework.
% \subsubsection{Item representation learning}

The introduction of the side information KG effectively help the generation of each item representation $e(v_i)$ in $P_{u^*}^t$, which involves in two aspects: the topology information of the global graph and the correlated semantic information of the sub-graph. Given entire knowledge graph, the representation of each entity can be learned by some general approaches such as TransE~\cite{bordes2013translating}. Such a pre-trained manner gives entities initial embeddings which effectively avoid the cold start problem. Then, since each item $v_i$ in the fake user profile are linked with entities in KG, then the representation of these items can be refined by taking advantages of the local semantics. Specifically, we employ graph transformer~\cite{shi2020masked} to recursively propagate neighbor semantic information along with the connectivity of entities. Moreover, the attention mechanism in graph transformer considers the diversity of the relations in KG by giving them different weights. More specifically, we first transform each item representation $e(v_i)$ by MLPs and then aggregate the weighted neighboring features of a given item representation $e(v_i)$:
\begin{equation}
    e^l(v_i) = W^g_1 e^{l-1}(v_i) + \sum_{v_j\in \mathcal{N}(v_i)}\alpha_{i,j} W^g_2 e^{l-1}(v_j)
\end{equation}
where $e^l(\cdot)$ denotes the embedding of an entity at layer $l$. $\mathcal{N}(\cdot)$ denotes the neighbors of an entity. $W^g_1$ and $W^g_2$ are two trainable parameters. The importance coefficients $\alpha_{i,j}$ are computed by:
\begin{equation}
    \alpha_{i,j} = \text{softmax}\Bigg( \frac{ \big( W^g_3e(v_i) \big)^{\top} \big( W^g_4e(v_j) \big) }{\sqrt{d}}  \Bigg)
\end{equation}
where $d$ is the node degree of $v_i$ in KG. $W^g_3$ and $W^g_4$ are two trainable parameters.

After getting all the item representations in the fake user profile, we aim to get the entire profile representation $e(s_t)$ which captures the attack intention of $P_{u^*}^t$. 
% Then, such a representation drives the DRL agent to learn a policy, which takes an action and outputs the user profile at time step $t+1$.
A general approach to finish this task is RNN since the user profile could be regarded as a time sequence. Then, to incorporate the historical information in $P_{u^*}^t$, in practice, we use RNN with GRU units to get the state representation $e(s_t)$ at time step $t$.
% Since items could be regarded as part of entities in KG, we can take advantage of the correlation structure in KG to generate an accurate embedding for each item.

% There are many embedding generating methods for KG~\cite{wang2018ripplenet,bordes2013translating}. Since the recommendation system is agnostic for the attacker, the task-specific embedding method such as RippleNet~\cite{wang2018ripplenet} is not appropriate for the black-box setting. Therefore, we utilize a general approach TransE~\cite{bordes2013translating} to generate initial embedding utilizing the structural information.

% As KG is a heterogeneous graph, the update of entity embedding via GNN should consider different relations importance. For better utilizing the structural and correlation information in KG, we employ graph transformer~\cite{shi2020masked} to recursively propagate neighbor semantic information along with the weighted connectivity of entities. Graph transformer contains two-part: node aggregation and node transformation. Specifically, in each layer of graph transformer, we first transform the entity embedding by MLPs and then aggregate the weighted neighboring features of a given item representation $e(v_t)$:
% \begin{equation}
%     e^l(v_t) = W^g_1 e^{l-1}(v_t) + \sum_{v_j\in \mathcal{N}(v_t)}\alpha_{t,j} W^g_2 e^{l-1}(v_j)
% \end{equation}
% where $e^l(\cdot)$ denotes the embedding of an entity at layer $l$. $\mathcal{N}(\cdot)$ denotes the neighbors of an entity. $W^g_1$ and $W^g_2$ are two trainable parameters. The importance coefficients $\alpha_{t,j}$ are computed by:
% \begin{equation}
%     \alpha_{t,j} = \text{softmax}\Bigg( \frac{ \big( W^g_3e(v_t) \big)^{\top} \big( W^g_4e(v_j) \big) }{\sqrt{d}}  \Bigg)
% \end{equation}
% where $d$ is the degree of $v_t$. $W^g_3$ and $W^g_4$ are two trainable parameters.
% However, using task-independent embeddings for GCN brings a cold-start problem, which may hinders the convergence of RL in the delay reward setting. To cope this problem, we pre-train the GNN by utilizing the unlabeled information in KG. Such a self-supervised manner can be formalized as:
% \begin{equation}
%     \text{here is GNN's auxillary loss function}
% \end{equation}

% \subsubsection{Profile representation learning layer}
% After getting all the item representations in the fake user profile, we aim to get the entire profile representation $e(s_t)$ which captures the attack intention of $P_{u^*}^t$. 
% % Then, such a representation drives the DRL agent to learn a policy, which takes an action and outputs the user profile at time step $t+1$.

% A general approach to finish this task is RNN since the user profile could be regarded as a sequence. Then, to incorporate the historical information in $P_{u^*}^t$, we use RNN with GRU unit to get the state embedding $e(s_t)$ at time step $t$:
% \begin{equation}
% \begin{aligned}
% &r_{t}=\sigma\left(W_{r} e(v_t)+U_{r} h_{t-1}+b_{r}\right) \\
% &u_{t}=\sigma\left(W_{u} e(v_t)+U_{u} h_{t-1}+b_{u}\right) \\
% &h_{t}=\tanh \left(W_c e(v_t)+U_c\left(r_{t} \cdot \hat{h}_{t-1}\right)+b_c\right) \\
% &e(s_t)=u_{t} \cdot h_{t-1}+\left(1-u_{t}\right) \cdot \hat{h}_{t} \\
% \end{aligned}
% \end{equation}
% where $r_t$ and $u_t$ denote the reset gate and update gate vector respectively. $h_t$ denotes the hidden state vector. $W$, $U$ and $b$ with subscripts denote the trainable parameters. Actually, more complicated entity embedding methods, GNN models and sequence representation methods could replace the adopted modules as mentioned above, and we leave this as a future work.

\subsection{Knowledge-enhanced Candidates Selection}
\label{Action candidates selection}





After having the state representation $e(s_t)$, \mymodel{} will select a new item from item candidate space and add it to the fake user profile at time step $t$. Incorporating KG brings two advantages towards the item candidates construction: First, it reduces the large search space. Selecting an item from the entire item space has $O(|V|)$ possible choices. The extremely large $|V|$ leads to the sample efficiency problem for DRL~\cite{zou2019reinforcement}. By utilizing structure of KG, we collect the neighbors of items $\{v_0,...,v_{t-1}\}$ in the user profile as the item candidates, which reduces the search space to $O(t|\mathcal{N}_v|)$, where $|\mathcal{N}_v|$ denotes the largest node degree of KG. Second, the item candidates incorporating the neighbor semantics further boost the effectiveness of promotion of the target item $v^*$, since reality users usually interact with items with similar semantic attributes.


% Next, we introduce the construction of the item candidates~(the action space). 
Specifically, given an item $v_i$ in the user profile, We first utilize KG to get its neighbor entities. We treat the neighbor entities~(entities could be item or non-item) as the seed set $\mathcal{E}_t^0$ at time step $t$. Then, the $H$-hop neighbor entity set is denoted as:
\begin{equation}
\begin{split}
    \mathcal{E}_t^l = \{ t|(h, r, t) \in \mathcal{G}, h\in \mathcal{E}_t^{l-1}  \},\\
    l=1,2,...,H
\end{split}
\end{equation}

As the fake user profiles are constructed by items, we only interested in the entities corresponding to the items. So the item candidates $\mathcal{C}_t$ is defined as:
\begin{equation}
\label{eq:candidates}
\mathcal{C}_t = \{ v|v\in \bigcup_{l=1}^H \mathcal{E}_t^{l}, v \in V  \}
\end{equation}


\subsection{Hierarchical Policy Network}
\subsubsection{Hierarchical Item Selection}

%In practice, the target item $v^*$ is usually unpopular (i.e., hardly appear in the Top-$k$ list of other users). It is possible that the neighbors of these unpopular items are also not in popular demand. Imagine an extreme case, the items in a user profile are all unpopular items. Then, it is difficult to expose the target item since the items in such a user profile have few interactions with other users.
Collecting neighbors of all the items in $P_{u^*}^t$ may dilute the action space and even harm the final attack performance.
% With the increases of the user profile length during profile generation, the size of action space would increase linearly if we consider the neighbors of all historical items in the profile as the item candidates. In addition, the neighbors of historical items in the profile may dilute the action space and even harm the final attack performance. 
To solve this problem, we adopt hierarchical action. Specifically, at time step $t$, the agent first performs $a_t^{(1)}$ to select an anchor item from $P_{u^*}^t$. We implement three types of anchor item selection strategies:
\begin{enumerate}
    \item Target:
    Since we aim to promote the target item, we believe that exploiting neighbors of the target item would boost the attack performance. Here, we set the target item as the anchor item.
    \item Tail:
    It is possible that the neighbors of the target item are deficient, which lead to inefficient structural utilization. On the other hand, exploring global items may also be beneficial. Therefore, for the second strategy, we utilize the tail item $v_{t-1}$ as the anchor item.
    
    % The pure exploitation of the target item may have a chance lead to bias. It is possible that the neighbors of the target item are deficient, which lead to inefficient structural utilization. On the other hand, the global items may also be beneficial. Therefore, for the second strategy, we utilize the tail item in the fake user profile being generated as the anchor item. In this way, the receptive field becomes large since the tail item are several hops away from the target item, and the agent have a chance to explore more global items in the entire item space.
    \item Dynamic:
    % The above two strategies considers two extreme case: pure exploitation of target item and pure exploration in the whole KG. By contrast, a more beneficial way is to 
    For the third strategy, we make a trade-off between exploitation and exploration, taking both target item and global items into consideration. Specifically, the agent will learn to perform action $a_t^{(1)}$ by a network to choose an anchor item from $P_{u^*}^t$ dynamically. In addition, we define an \emph{anchor ratio} $\epsilon$ to speed up the policy learning. The anchor ratio denotes the probability the agent explores the global items. Large $\epsilon$ encourages the agent to select an anchor item from any item in $P_{u^*}^t$, while low $\epsilon$ forces the agent to select the target item as the anchor item.
    
    % Specifically, at time step $t$, the agent would learn to perform action $a_t^{(1)}$ to select an anchor from $t$ historical items in the fake user profile. \red{anchor ratio}
\end{enumerate}
%\paragraph{Item picking}
Then, the agent performs action $a_t^{(2)}$ to pick a new item from the neighbors of anchor item, and adds this item to $P_{u^*}^t$ at time step $t$. 

The item candidates constructed based on the anchor item are believed to be promising. Moreover, the hierarchical action enables the size of item candidates to be independent of the length of the fake user profile. The process of hierarchical action is illustrated in Figure~{\red{?}}. As a result, with the hierarchical action $a_t = (a_t^{(1)},a_t^{(2)})$, the trajectory of the proposed MDP is $(s_0,a_0^{(1)},a_0^{(2)},r_0,...,s_{T-1},a_{T-1}^{(1)},a_{T-1}^{(2)},r_{T-1},s_T)$


\subsubsection{Hierarchical Policy Network}
We adopt the A2C architecture~\cite{mnih16asy} which is widely used in RL algorithms to learn the best policy. A2C usually has one actor network and one critic network. The critic network is used to estimate the state-value function $V(s_t)$ which measures the expected attack performance start at state $s_t$, while the actor network is used to choose the action given the current state $s_t$. For hierarchical action space, we utilize two actor networks to perform two level actions separately: One actor network learns a stochastic policy $\pi^{(1)}(a_t^{(1)}|s_t)$ to select the anchor item and the other actor network learns a stochastic policy $\pi^{(2)}(a_t^{(2)}|s_t)$ to pick an item from the item candidates constructed based on the anchor item. The outputs of the actor network is the probability of each possible action. Then, action $a_t = (a_t^{(1)},a_t^{(2)})$ will be sampled to steer the RL agent. 


Specifically, after obtaining the state representation $e(s_t)$ at time step $t$, the agent first performs the action $a_t^{(1)}$ sampled from $ [p_{t,0},...,p_{t,t-1}] \in [0,1]^t$, which is a $t$-length probability vector indicating the possibility of each item $v_i$ to be the anchor item in the fake user profile. However, such an probability vector whose length changes with $t$ brings difficulties for the actor network to output. That is, at each time step $t$, only $t$ historical items in $P^t_{u^*}$ are valid anchor item candidates. To avoid giving an invalid action, we utilize the mask technique to manage the first level action space~\cite{huang2020closer}.

More specifically, given $e(s_t)$, the action $a_t^{(1)}$ are sampled according to:
\begin{equation}
\begin{split}
    H_t = &\text{RELU}(W_1e(s_t)+b_1)\\
    \hat{H}_t =& W_2H_t + m_t\\
    \pi_{\Theta_1}^{(1)}(a_t^{(1)}|s_t)=&\frac{exp(\hat{H}_t^i)}{\sum_{j=0}^{T-1} exp(\hat{H}_t^j) },i=0,...,T-1
\end{split}
\end{equation}
where $\Theta_1=\{W_1 \in \mathbb{R}^{h_1 \times h_s}, W_2 \in \mathbb{R}^{T \times h_1}, b_1 \in \mathbb{R}^{h_1} \}$ are the learnable weights. $h_s$ denotes the dimension of the embedding size of $e(s_t)$, and $h_1$ denotes the dimension of the hidden layer. $\hat{H}_t$ denotes the masked $T$ length logits vector $\hat{H}_t=[\hat{H}_t^0...,\hat{H}_t^{T-1}]$, and $m_t$ denotes the length $T$ mask vector at time step $t$, which modifies the logits to assign large negative value to invalid actions:
\begin{equation}
\begin{split}
m^i_{t}=
\begin{cases}
0& 0<i<t\\
-\infty& t\leq i<T
\end{cases}    
\end{split}
\end{equation}

In this way, the probability of sampling the invalid anchor item will be $0$.

Once the first action $a_t^{(1)}$ are sampled, the second level action space $\mathcal{C}_t$ will be determined. Then, we utilize the second actor network to compute the probability of each item in $\mathcal{C}_t$:

%the agent sample the second action $a_t^{(2)}$ based on the generated item candidates set $\mathcal{C}_t$ as:
\begin{equation}
\begin{split}
    H_t = \text{RELU}&(W_3e(s_t)+b_2)\\
    \pi_{\Theta_2}^{(2)}(a_t^{(2)}|s_t)) =& \frac{exp(W_4[H_t||e(v_t)])}{\sum_{v_t\in\mathcal{C}_t}exp(W_4 [H_t||e(v_t)])}
    \end{split}
\end{equation}
where $\Theta_2=\{W_3 \in \mathbb{R}^{h_2 \times h_s},W_4 \in \mathbb{R}^{h_2+h_a}, b_2 \in \mathbb{R}^{h_2}$\} are the learnable weights. $h_a$ denotes the embedding size of $e(v_t)$, and $h_2$ denotes the dimension of the hidden layer.
% \Pi\theta^{(1)}= 
% state representation [B*H] T parameter vector [T*H] ---> [B*T] \in (0,1)
% \Pi \theta^{(2)}=:
% state representation [B*H]  [B*C*H]
\subsubsection{Model Training}
% loss function
We aim at finding the optimal parameters of the policy network to maximize the expected return $\mathbb{E}_{\tau \sim \{\pi_{\Theta_1},\pi_{\Theta_2} \}} R(\tau)$,
% \begin{equation}
%     \Theta^* = \{\Theta_1^*,\Theta_2^*\} = \text{argmax}_{\Theta}\sum_\tau p_{\Theta}(\tau;\Theta)R(\tau) 
% \end{equation}
where $\tau$ denotes an injected $T$-length fake user profile $P_{u^*}$~(trajectory), $R(\tau)$ is the discounted return and is calculated as $R(\tau) = \sum_{t=0}^{T-1} \gamma^t r(s_t,a_t)$. In practice, we get reward after we inject $N$ trajectories simultaneously, and we set $R(\boldsymbol{\tau})$ the same for each injected trajectory $\tau$ in $\boldsymbol{\tau}$, where $\boldsymbol{\tau}$ denotes a set of $T$-length fake user profile $P_{u^*}$ with set size $N$.

% we note that $\boldsymbol{\tau}$ denotes a set of $T$-length fake user profile $P_{u^*}$ with set size $N$. Since we calculate Hit Ratio after we inject $N$ trajectories, we set $R(\boldsymbol{\tau})$ the same for each injected trajectory $\tau$ in specific $\boldsymbol{\tau}$.

% gradient of the profile refine policy function
For hierarchical RL training, we adopt PPO~\cite{schulman2017proximal} to update the first actor network by minimize the following objective:
\begin{equation}
\label{gradient}
\begin{split}
    L({\Theta_1}) = \frac{1}{T}\sum_{t=0}^{T-1} 
    \min\Big(\frac{p_{\Theta_1}(a_t^{(1)}|s_t)}{p_{\Theta_1'}(a_t^{(1)}|s_t)}\hat{A}_t,\\
    \text{clip}(\frac{p_{\Theta_1}(a_t^{(1)}|s_t)}{p_{\Theta_1'}(a_t^{(1)}|s_t)},1-\phi,1+\phi)\hat{A}_t \Big)
\end{split}
\end{equation}
where $p_{\Theta_1}(a_t^{(1)}|s_t)$ and $p_{\Theta_1'}(a_t^{(1)}|s_t)$ are the probabilities given by $\pi^{(1)}(a_t^{(1)}|s_t)$ under the current parameters $\Theta_1$ and the old parameters $\Theta_1'$. $\phi$ is the hyperparameter used to clip the probability ratio defined in PPO. $\hat{A}_t$ is the variance reduced advantage function estimator defined in PPO, which is calculated based on $V(s)$ and $R(\tau)$.
%We sample $N$ trajectory set $\boldsymbol{\tau}$ and calculate the gradient for the first policy network $\pi^{(1)}(a_t^{(1)}|s_t)$
% gradient of the candidate select policy function
The objective function for the second policy network $\pi^{(2)}(a_t^{(2)}|s_t)$ is calculated in the same way. The training process is shown in Algorithm 1.
\begin{algorithm}
\caption{Training process for hierarchical policy network }
\textbf{Input} Fake user number $N$, trajectory length $T$      \\
\textbf{Output} The learned policy network $\pi_{\Theta_1}$,$\pi_{\Theta_2}$\\
\begin{algorithmic}[1]
% \Procedure{Traininig}{$\pi_{\Theta_1}$,$\pi_{\Theta_2}$,$B$,$T$,$N$}
\STATE Initialize the parameters in the policy network
\STATE Initialize replay memory buffer $\mathcal{B}$
% \FOR{$v^* \in V$}
\FOR{$ budget \gets 1,2,...,\Delta$}
% \FOR{$n\gets 1,2,...,N$}
\FOR{$t\gets 0,1,...,T-1$}
\STATE Sample $a_t^{(1)}$ by $\pi_{\Theta_1}$
\STATE Generate the item candidate set $\mathcal{C}_t$ according to  $a_t^{(1)}$
\STATE Sample $a_t^{(2)}$ by $\pi_{\Theta_2}$
\STATE Set $s_{t+1} = \{s_t,a_t^{(2)}\}$
\STATE Collect $\{a_t^{(1)}, p(a_t^{(1)}|s_t), a_t^{(2)}, p(a_t^{(2)}|s_t), s_{t+1}, r_t, \mathcal{C}_t\}$ in memory buffer $\mathcal{B}$
% \ENDFOR
\ENDFOR
% \STATE Inject N fake user profiles to the target system and get reward $r$, and assign $r$ for every $N$ trajectory,
% \STATE Compute $R(\tau)_t$, $V(s_t)$, $\hat{A}_t$ at each step $t$ based on $\matchcal{B}$
\STATE update parameters of two actor networks and one critic network by maximizing Equation~\ref{gradient}
\STATE clean memory buffer $\mathcal{B}$
\ENDFOR
% \ENDFOR

\end{algorithmic}
\end{algorithm}


% \end{document}

==> sections/model3.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}

% % \begin{document}




\subsection{Overview of KGAttack}




\begin{figure}[ht]
\centering
\centerline{\includegraphics[width=\columnwidth]{images/KGAttack-Framework.drawio.png}}
\caption{An overview of the proposed framework \mymodel{}. \red{need to be updated before submission!  [Knowledge-enhanced Candidate Selection]}}
%\mymodel{} consists of four major components: state representation learning, candidates construction, hierarchical policy network, and injection attack and queries
% \red{it would be better if we can explicitly show  profile representation learning, candidates construction, pivot selection, item picking, and injection attack and queries in the figure.}
\label{fig:farmework}
\end{figure}

\begin{figure}[ht]
\centering
\centerline{\includegraphics[width=0.9\columnwidth]{images/KGAttack-four modules.drawio.png}}
\caption{A detailed illustration of four major components of KGAttack: knowledge-enhanced state representation learning, knowledge-enhanced candidates construction, hierarchical policy network, and injection attack and queries.}
% \red{it would be better if we can explicitly show  profile representation learning, candidates construction, pivot selection, item picking, and injection attack and queries in the figure.}
\label{fig:KGAttack_components}
\end{figure}
%To address the problem of black-box recommendation system attacking, we propose a reinforcement learning~(RL) based method, \mymodel{}. 


To attack a target recommender system under black-box setting,  we introduce a knowledge graph-enhanced reinforcement learning  based attacking framework (\mymodel{}) to learn a  strategy of generating fake user profile and interact with the black-box system.
The architecture of our proposed attacking framework (\mymodel{}) is shown in Figure~\ref{fig:farmework}. The framework consists of four major components: knowledge-enhanced state representation learning, knowledge-enhanced candidate construction, hierarchical policy networks, and injection attack and queries.
Knowledge-enhanced state representation learning aims to learn the representations of generated fake user profiles (i.e., a set of items) with knowledge graph-enhanced at state $t$.  Knowledge-enhanced candidate construction is to leverage the knowledge graph to obtain relevant item candidates (i.e., action pool).  Hierarchical policy networks aim to learn a strategy for selecting potential items for user profile generations. Injection attack and queries perform attacking with query feedback to update the policy. Next we discuss the details for each component.


\subsection{Knowledge-enhanced State Representation Learning}

The component of knowledge-enhanced state representation learning is illustrated in Figure~\ref{fig:KGAttack_components}.
Given a fake user profile $P_{u^*}^t = \{v_0,..., v_*,...,v_{t-1} \}$ for attacking (i.e., promoting) a target item  $v*$ at state $t$, knowledge-enhanced state representation learning aims to learn the representations of fake user profiles $\mathbf{x}_{u_i}^t$, which is crucial to learn the optimal attacking strategy in reinforcement learning. In order to take advantage of semantic and correlation information among items, knowledge graph is incorporated to enhance  representation learning of user profiles $P_{u^*}^t $. However, utilizing the knowledge graph into learning profile representation is rather challenging since the knowledge graph is heterogeneous with comprehensive information. 

\noindent \textbf{Knowledge-enhanced State Representation.} To address this challenge, we propose to utilize graph neural networks (GNNs) to learn representation for each item in user profile. The intuition of using GNNs can naturally model node feature and topological structure  by using deep neural networks\red{[]}.  Mathematically, an aggregation operation of GNNs to learn knowledge-enhanced item representations can be defined as follows:
\begin{equation}
     \mathbf{e}^{l}_i = \mathbf{W}^{l}_1  \cdot \mathbf{e}^{l-1}_i + \mathbf{W}^{l}_2 \cdot \sum_{v_j\in \mathcal{N}(v_i)}\alpha_{i,j}  \mathbf{e}_j^{l-1}
\end{equation}
where $\mathbf{e}^{l}_i$ denotes the embedding of an entity $v_i$ (i.e., item or non-item) at layer $l$, and $\mathcal{N}(v_i)$ denotes the neighbors of an entity $v_i$. $\mathbf{W}^l_1$ and $\mathbf{W}^l_2$ are  trainable weights at layer $l$.  Moreover, we introduce a relation attention  to characterize different relationships between entities in heterogeneous graph as follows:
\begin{equation}
    \alpha_{i,j} = \text{softmax}\Bigg(  \big( \mathbf{W}^{in}  \cdot \mathbf{e}^{l-1}_i \big)^{\top} \big(  \mathbf{W}^{out}  \cdot \mathbf{e}^{l-1}_j   \big) /\sqrt{d}  \Bigg)
\end{equation}
where $\alpha_{i,j}$ denotes the  importance coefficients $\alpha_{i,j}$ between entity $v_i$ and entity $v_j$ at layer $l$. $\mathbf{W}^{in} $ and $\mathbf{W}^{out} $ are trainable weights.

Additionally, TransE~\cite{bordes2013translating}, one of the representative techniques for knowledge graph embedding, is used to pre-train entities (i.e., item and non-item) and relations as embedding vectors as the input of GNNs. More specifically,  $\mathbf{e}^{0}_i$ is initialized through optimizing objective function as follows:
\red{TransE}.
 \begin{equation}
 L = \sum_{(h,r,t) \in \mathcal{S}_+}\sum_{(h',r',t')\in \mathcal{S}^-} [ f_r(h,t) + \phi - f_r(h^',t^') ]
%      L = \sum_{(h,r,t) \in \matccal{S}_+}\sum_{(h',r',t')\in \matchcal{S}^-} [f_r(h,t) + \phi - f_r(h^',t^')]_+
 \end{equation}
%The representation $\mathbf{e}^{l}_i$ at final layer of GNNs can be denoted as the knowledge-enhanced item representation.

For simplicity, the final knowledge-enhanced item representation is denoted as  $\mathbf{e}_i$. 


\noindent \textbf{State Representation learning.} Since user profiles contain sequential dependency (i.e., long and short term), it is natural to  employ a Recurrent Neural Network (RNN) model to encode fake user profiles as low-dimensional representation. Thus, we adopt a RNN with a gated recurrent unit (GRU) as the network cell \red{[]} to capture fake user's historical behaviors based on the knowledge-enhanced item representation as follows:

\red{Please illustrate how GRU works here!}
\begin{equation}
       \mathbf{x}^{t}_{u^*} = \text{RNN} (P_{u^*}^t)
\end{equation}




\subsection{Knowledge-enhanced Candidate Selection}
\label{Action candidates selection}





% Once having the embedding of each item in the fake user profile, \mymodel{} aims to add an item to the profile sequentially to make the profile complete. However, directly selecting an item from the entire item candidates space has $O(|V|)$ possible choices. The extremely large $|V|$ leads to the sample efficiency problem for DRL~\cite{zou2019reinforcement}. To reduce the item candidates, in \emph{Candidate Construction} module, we construct the item candidates based on the correlation structure of KG. Specifically, we obtain the item candidates by collecting the neighbors of historical items in the profile being generated.
%Such correlated information not only reduces the search space but also alleviates the cold start problem.
After getting the state representation $e(s_t)$, \mymodel{} will select a new item from item candidate space and add it to the fake user profile at time step $t$. Incorporating KG brings two advantages towards the item candidates construction: First, it reduces the large search space. Selecting an item from the entire item space has $O(|V|)$ possible choices. The extremely large $|V|$ leads to the sample efficiency problem for DRL~\cite{zou2019reinforcement}. By utilizing structure of KG, we collect the neighbors of items $\{v_0,...,v_{t-1}\}$ in the user profile as the item candidates, which reduces the search space to $O(t|\mathcal{N}_v|)$, where $|\mathcal{N}_v|$ denotes the largest node degree of KG. Second, the item candidates incorporating the neighbor semantics further boost the effectiveness of promotion of the target item $v^*$, since reality users usually interact with items with similar semantic attributes.

% selecting the neighbors of items in the user profile makes the user profile similar to real ones. In reality, users usually interact with items with similar semantic information, while the items linked in the KG satisfy such a similar characteristic.

% Next, we introduce the construction of the item candidates~(the action space). 
Specifically, given an item $v_i$ in the user profile, We first utilize KG to get its neighbor entities. We treat the neighbor entities~(entities could be item or non-item) as the seed set $\mathcal{E}_t^0$ at time step $t$. Then, the $H$-hop neighbor entity set is denoted as:
\begin{equation}
\begin{split}
    \mathcal{E}_t^l = \{ t|(h, r, t) \in \mathcal{G}, h\in \mathcal{E}_t^{l-1}  \},\\
    l=1,2,...,H
\end{split}
\end{equation}

As the fake user profiles are constructed by items, we only interested in the entities corresponding to the items. So the item candidates $\mathcal{C}_t$ is defined as:
\vspace{-0.1cm}
\begin{equation}
\label{eq:candidates}
\mathcal{C}_t = \{ v|v\in \bigcup_{l=1}^H \mathcal{E}_t^{l}, v \in V  \}
\end{equation}



\subsection{Hierarchical Policy Network}



\subsubsection{Hierarchical Item Selection}
 
Collecting neighbors of all the items in $P_{u^*}^t$ may dilute the search space and even harm the final attack performance.
% With the increases of the user profile length during profile generation, the size of action space would increase linearly if we consider the neighbors of all historical items in the profile as the item candidates. In addition, the neighbors of historical items in the profile may dilute the action space and even harm the final attack performance. 
To solve this problem, we adopt hierarchical actions. Specifically, at time step $t$, the agent first performs $a_t^{(1)}$ to select an anchor item from $P_{u^*}^t$ to refine the item candidates. We believe that the neighbors of anchor item can construct promising item candidates. We implement three types of anchor item selection strategies:
\begin{itemize}
    \item \textbf{Target}:
    Exploiting neighbors of the target item $v^*$ as item candidates. Here, we set $v^*$ as the anchor item.
    \item \textbf{Global}:
    It is possible that the neighbors of the target item are deficient, which leads to inefficient structural utilization. Also, exploring global items may be beneficial. Therefore, for the second strategy, we utilize the last item $v_{t-1}$ in the current profile as the anchor item.
    
    % The pure exploitation of the target item may have a chance lead to bias. It is possible that the neighbors of the target item are deficient, which lead to inefficient structural utilization. On the other hand, the global items may also be beneficial. Therefore, for the second strategy, we utilize the tail item in the fake user profile being generated as the anchor item. In this way, the receptive field becomes large since the tail item are several hops away from the target item, and the agent have a chance to explore more global items in the entire item space.
    \item \textbf{Mix}:
    % The above two strategies considers two extreme case: pure exploitation of target item and pure exploration in the whole KG. By contrast, a more beneficial way is to 
    For the third strategy, we make a trade-off between target exploitation and global exploration. We define an \emph{anchor ratio} $\epsilon$ to achieve such trade-off. 
    % Specifically, the agent will learn to perform action $a_t^{(1)}$ by a network to .  
    The agent has $\epsilon$ probability to learn to choose an anchor item from $P_{u^*}^t$ by a policy, while has $1-\epsilon$ probability to set the target item as anchor item. 
    % Here, large $\epsilon$ encourages the agent to explore an anchor item in $P_{u^*}^t$.
    
    % Specifically, at time step $t$, the agent would learn to perform action $a_t^{(1)}$ to select an anchor from $t$ historical items in the fake user profile. \red{anchor ratio}
\end{itemize}
%\paragraph{Item picking}
As a result, the anchor item refines the item search space and enables the size of item candidates to be independent of the length of the fake user profile. Then, the agent performs action $a_t^{(2)}$ to pick a new item from the refined item candidates, and adds this item to $P_{u^*}^t$. The process of hierarchical action is illustrated in the top-right part of Figure~\ref{fig:KGAttack_components}. 


\subsubsection{Hierarchical Policy Network}
%hierarchical policy network 的motivation --> hierarchical actions
% Due to the sparse reward~(we get reward after injecting the complete length $T$ fake user profile), 
To achieve the hierarchical actions, we adopt the A2C architecture~\cite{mnih16asy} which is widely used in RL algorithms. A2C usually has one actor network and one critic network. The critic network is used to estimate the state-value function $V(s_t)$ which measures the expected rewards start at state $s_t$, while the actor network is used to choose the action. For hierarchical actions, we utilize two actor networks separately: One actor network learns a stochastic policy $\pi^{(1)}(a_t^{(1)}|s_t)$ to select the anchor item and the other learns a stochastic policy $\pi^{(2)}(a_t^{(2)}|s_t)$ to pick an item from the item candidates. 

Specifically, after obtaining the state representation $e(s_t)$, the agent first performs the action $a_t^{(1)}$ sampled from 
% $ [p_{t,0},...,p_{t,t-1}] \in [0,1]^t$, which is 
a $t$-length probability vector indicating the possibility of each item $v_i$ to be the anchor item. However, at each time step $t$, only $t$ historical items in $P^t_{u^*}$ are valid anchor item candidates. Such varying action space brings difficulties for the actor network to output. To avoid giving an invalid action, we utilize the mask technique to manage the first level action space~\cite{huang2020closer}.

More specifically, given $e(s_t)$, the action $a_t^{(1)}$ are sampled according to:
\vspace{-0.2cm}
\begin{equation}
\begin{split}
    \hat{H_t} = &W_2\text{RELU}(W_1e(s_t)+b_1)+m_t\\
    % \hat{H}_t =& W_2H_t + m_t\\
    \pi_{\Theta_1}^{(1)}(a_t^{(1)}|s_t)=&\frac{exp(\hat{H}_t^i)}{\sum_{j=0}^{T-1} exp(\hat{H}_t^j) },i=0,...,T-1
\end{split}
\end{equation}
where $\Theta_1=\{W_1 \in \mathbb{R}^{h_1 \times h_s}, W_2 \in \mathbb{R}^{T \times h_1}, b_1 \in \mathbb{R}^{h_1} \}$ are the learnable weights. $h_s$ denotes the embedding size of $e(s_t)$, and $h_1$ denotes the hidden layer dimension. $\hat{H}_t$ denotes the masked $T$ length logits vector
% $\hat{H}_t=[\hat{H}_t^0...,\hat{H}_t^{T-1}]$, 
and $m_t$ denotes the mask vector at time step $t$, which modifies the logits to assign large negative value to invalid actions.
% \begin{equation}
% \begin{split}
% m^i_{t}=
% \begin{cases}
% 0& 0<i<t\\
% -\infty& t\leq i<T
% \end{cases}    
% \end{split}
% \end{equation}
In this way, the probability of sampling the invalid anchor item will be $0$.

Once the first level action $a_t^{(1)}$ are sampled, the second level action space $\mathcal{C}_t$ will be determined. Then, we utilize the second actor network to compute the probability of each item in $\mathcal{C}_t$:
\vspace{-0.2cm}
%the agent sample the second action $a_t^{(2)}$ based on the generated item candidates set $\mathcal{C}_t$ as:
\begin{equation}
\begin{split}
    H_t = \text{RELU}&(W_3e(s_t)+b_2)\\
    \pi_{\Theta_2}^{(2)}(a_t^{(2)}|s_t)) =& \frac{exp(W_4[H_t||e(v_t)])}{\sum_{v_t\in\mathcal{C}_t}exp(W_4 [H_t||e(v_t)])}
    \end{split}
\end{equation}
where $\Theta_2=\{W_3 \in \mathbb{R}^{h_2 \times h_s},W_4 \in \mathbb{R}^{h_2+h_a}, b_2 \in \mathbb{R}^{h_2}$\} are the learnable weights. $h_a$ denotes the embedding size of $e(v_t)$, and $h_2$ denotes the dimension of the hidden layer.
% \Pi\theta^{(1)}= 
% state representation [B*H] T parameter vector [T*H] ---> [B*T] \in (0,1)
% \Pi \theta^{(2)}=:
% state representation [B*H]  [B*C*H]


\subsection{Injection Attack and Queries}

\subsection{Attacking Environment}
The black-box attacking process can be formulated as a Markov decision process~(MDP) $\mathcal{<S,A,P}, r,\gamma>$ . The definition of MDP contains state space $\mathcal{S}$, action space $\mathcal{A}$, transition probability $P$, reward $r$, and discount factor $\gamma$:
\begin{itemize}
    \item State: The state $s_t \in \mathcal{S}$ is abstracted from the fake user profile $P_{u^*_i}^t=\{v_0 \rightarrow...\rightarrow v_{t-1}\}$ at time step $t$.
    \item Action: The action $a_t = \{a^{(1)}_t,a^{(2)}_t\} \in \mathcal{A}$ has two components. Specifically, at each time step $t$, the agent first performs the action $a_t^{(1)}$ to select an anchor item from $P_{u^*_i}^t$, then performs the action $a_t^{(2)}$ to pick a new item from the refined item candidates.
    % \item Transition probability: The state transition function $p(s_{t+1}|s_t,a_t) \in \mathcal{P}:\mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S} $ defines the probability of state transition from $s_t$ to $s_{t+1}$ when the attacker takes an action $a_t$.
    \item Reward: 
    % As the attacker aims to promote the target item $v^*$ that can be appeared in the Top-$k$ recommendation list of other users, we use the 
    Hit Ratio~(HR@K), a ranking evaluation metric, is used as the reward function $r(s_t,a_t)$, which is defined as follows:
    \vspace{-0.2cm}
    \begin{equation}
    \begin{split}
    r(s_t,a_t) &= 
        \begin{cases}
        \sum^{|\hat{U}|}_{i=1} \text{HR}(\hat{u}_i, v^*, k)& t=T-1\\
        0& \text{otherwise}
        \end{cases}
         \\
    &\text{HR}(\hat{u}_i, v^*, k) =
    \begin{cases}
    1&v^* \in y_{\hat{u}_i,>k}\\
    0&v^* \notin y_{\hat{u}_i,>k}
    \end{cases}
    \end{split}
    \end{equation}
    where $\text{HR}(\hat{u}_i, v^*, k)$ returns the hit ratio for a target item $v^*$ in the top-$k$ list of the spy user $\hat{u}_i \in \hat{U}$. Here, the set of spy users $\hat{U}$ can be a subset of normal users who are already established in the target recommender system before the injection attack. 
    They can be used by the attacker as a measure of promotion effectiveness of the injected fake users' profiles. 
    % We calculate the HR of each spy users after injecting the complete fake user profile with length $T$.
    \item Terminal: The attacking process will stop if the number of entire injected user profiles reaches the budget $\Delta$.
    
\end{itemize}


\subsubsection{Model Training}
% loss function
We aim to train the policy network to maximize the expected return $\mathbb{E}_{\tau \sim \{\pi_{\Theta_1},\pi_{\Theta_2} \}} R(\tau)$,
% \begin{equation}
%     \Theta^* = \{\Theta_1^*,\Theta_2^*\} = \text{argmax}_{\Theta}\sum_\tau p_{\Theta}(\tau;\Theta)R(\tau) 
% \end{equation}
where $\tau$ denotes an injected $T$-length fake user profile $P_{u^*}$~(trajectory), $R(\tau)$ is the discounted return and is calculated as $R(\tau) = \sum_{t=0}^{T-1} \gamma^t r(s_t,a_t)$. In practice, we get the reward after injecting $N$ profiles and set the reward the same for each injected profile.
% we set $R(\boldsymbol{\tau})$ the same for each injected trajectory $\tau$ in $\boldsymbol{\tau}$, where $\boldsymbol{\tau}$ denotes a set of $T$-length fake user profile $P_{u^*}$ with set size $N$.

% we note that $\boldsymbol{\tau}$ denotes a set of $T$-length fake user profile $P_{u^*}$ with set size $N$. Since we calculate Hit Ratio after we inject $N$ trajectories, we set $R(\boldsymbol{\tau})$ the same for each injected trajectory $\tau$ in specific $\boldsymbol{\tau}$.

% gradient of the profile refine policy function
For hierarchical RL training, we adopt PPO~\cite{schulman2017proximal} to update the first actor network by minimize the following objective:
\vspace{-0.2cm}
\begin{equation}
\label{gradient}
\begin{split}
    L({\Theta_1}) = \frac{1}{T}\sum_{t=0}^{T-1} 
    \min\Big(\frac{p_{\Theta_1}(a_t^{(1)}|s_t)}{p_{\Theta_1'}(a_t^{(1)}|s_t)}\hat{A}_t,\\
    \text{clip}(\frac{p_{\Theta_1}(a_t^{(1)}|s_t)}{p_{\Theta_1'}(a_t^{(1)}|s_t)},1-\phi,1+\phi)\hat{A}_t \Big)
\end{split}
\end{equation}
where $p_{\Theta_1}(a_t^{(1)}|s_t)$ and $p_{\Theta_1'}(a_t^{(1)}|s_t)$ are the probabilities given by $\pi^{(1)}(a_t^{(1)}|s_t)$ under the current parameters $\Theta_1$ and the old parameters $\Theta_1'$. $\phi$ is the hyperparameter used to clip the probability ratio. $\hat{A}_t$ is the variance reduced advantage function estimator, which is calculated based on $V(s)$ and $R(\tau)$.
%We sample $N$ trajectory set $\boldsymbol{\tau}$ and calculate the gradient for the first policy network $\pi^{(1)}(a_t^{(1)}|s_t)$
% gradient of the candidate select policy function
The objective function for the second actor network $\pi^{(2)}(a_t^{(2)}|s_t)$ is formulated in the same way. The training algorithm of hierarchical policy network is provided in the supplementary material.


==> sections/problem.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}

% \begin{document}
\subsection{Problem Statement and Notations}
%介绍推荐系统本身
Let $U = \{u_1,...,u_m \}$ and $V = \{ v_1,...,v_n\}$ be the sets of users and items in  target recommender system, respectively. The user-item interactions  can be defined as matrix $\mathbf{Y}\in \mathbb{R}^{m\times n}$,  where $y_{ij} = 1$ indicates that user $u_i$ has interacted with item $v_j$~(e.g., clicked/watched), and $0$ otherwise.
The user profile $P_{u_i} = \{v_0,...,v_{l-1}\}$ is defined as $l$ historical items the user $u_i$ interacted with in $\mathbf{Y}$~($l$ can vary between users). 
% where $\rightarrow$ denotes the sequential order. 
% After that, the set of all user profiles can be denoted as $P_U = \{ P_{u_1},...,P_{u_m} \}$. 
In addition, in real-life application, items' external knowledge (i.e., attributes) can be accessed and formulated as knowledge graph (KG~ $\mathcal{G}$) comprised of entity-relation-entity triples  $(p,r,q)$. Here, entities $p,q\in \mathcal{E}$ denote the head and tail of a triple respectively, and $r \in \mathcal{R}$ denotes the relation. For instance, the triple (\textit{Avatar, film.film.director, James Cameron}) states the fact that \emph{James Cameron} is the director of the film \emph{Avatar}. 
The goal of the target recommender system is to predict whether user $u_i$ will interact with an item $v_j$ via generating a top-$k$ ranked potential items $y_{i,>k} = \{v_{[1]},...,v_{[k]} \}$ for user $u_i$, where user $u_i$ is more likely to interact with $v_{[i]}$ than $v_{[i+1]}$. 


The task of black-box attacks is to promote a target item $v^* \in V $ by generating a set of fake users $U^* = \{u_i^*\}_{i=1}^\Delta$ with their profiles $P_{u_i}$ and inject them into user-item interactions $Y$, where $\Delta$ is the budget given to the attacker. This results in the target system having a set of polluted users $U' = U \cup U^*$ and a polluted interaction matrix $Y'\in \mathbb{R}^{(\Delta+m )\times n}$. The promotion of a target item $v^*$ is to have the $v^*$ recommended to users in $U$ that did not have $v^*$ appeared in their Top-$k$ recommendation list before attacks.


